Study of a giant Large Magellanic Cloud Supernova Remnant, Veliki (J0450.4-7050)

We present a high-resolution radio-continuum view and a multi-frequency analysis of the Large Magellanic Cloud (LMC) Supernova Remnant (SNR) J0450.4-7050, which we give the nickname Veliki. These high-resolution observations reveal a larger extent than previously measured, making J0450.4-7050 one of the largest SNRs that we know of. Additionally, we observe a higher than expected radio surface brightness and an unusually flat spectral index ($\alpha = -0.26 \pm 0.02$), with little spectral variation over the remnant. We observe a bright H$\alpha$ shell indicating significant cooling over the remnant, but also an excess of [Oiii] on the eastern shock front. We investigate several theoretical scenarios to explain the emission and radio evolution of J0450.4-7050 in the context of the LMC environment, and determine that this is most likely an older, predominantly radiative, SNR with a higher shock compression ratio, which gives a flatter non-thermal spectrum, in combination with a thermal (bremsstrahlung) emission contribution.

==> abr_saj.tex <==
\newcommand\aap{A\&A}%
\newcommand\aapr{A\&ARv}%
\newcommand\aaps{A\&AS}%
\newcommand\aas{AAS Meeting Abstracts}%
\newcommand\actaa{AcA}%
\newcommand\aj{AJ}%
\newcommand\ao{ApOpt}%
\newcommand\apj{ApJ}%
\newcommand\apjl{ApJL}     %
\newcommand\apjs{ApJS}%
\newcommand\aplett{Astrophys.~Lett.}%
\newcommand\apspr{Astrophys.~Space~Phys.~Res.}%
\newcommand\apss{Ap\&SS}%
\newcommand\araa{ARA\&A}%
\newcommand\azh{AZh}%
\newcommand\baas{BAAS}%
\newcommand\bac{Bull. astr. Inst. Czechosl.}
\newcommand\bain{BAN}%
\newcommand\caa{ChA\&A}%
\newcommand\cjaa{ChJA\&A}%
\newcommand\dps{AAS/DPS Meeting Abstracts}%
\newcommand\fcp{FCPh}%
\newcommand\gca{GeoCoA}%
\newcommand\grl{Geophys.~Res.~Lett.}%
\newcommand\iaucirc{IAUC}%
\newcommand\icarus{Icar}%
\newcommand\jcap{JCAP}%
\newcommand\jcp{JChPh}%
\newcommand\jgr{JGR}%
\newcommand\jqsrt{JQSRT}%
\newcommand\jrasc{JRASC}%
\newcommand\maps{M\&PS}%
\newcommand\memras{MmRAS}%
\newcommand\memsai{MmSAI}%
\newcommand\mnras{MNRAS}%
\newcommand\na{NewA}%
\newcommand\nar{NewAR}%
\newcommand\nat{Natur}%
\newcommand\nphysa{NuPhA}%
\newcommand\pasa{PASA}%
\newcommand\pasj{PASJ}%
\newcommand\pasp{PASP}%
\newcommand\physrep{PhR}%
\newcommand\physscr{PhyS}%
\newcommand\planss{Planet.~Space~Sci.}%
\newcommand\pra{PhRvA}%
\newcommand\prb{PhRvB}%
\newcommand\prc{PhRvC}%
\newcommand\prd{PhRvD}%
\newcommand\pre{PhRvE}%
\newcommand\prl{PhRvL}%
\newcommand\procspie{Proc.~SPIE}%
\newcommand\qjras{QJRAS}%
\newcommand\rmxaa{RMxAA}%
\newcommand\skytel{S\&T}%
\newcommand\solphys{SoPh}%
\newcommand\sovast{Soviet~Ast.}%
\newcommand\ssr{SSRv}%
\newcommand\zap{ZA}%

\let\astap=\aap 
\let\apjlett=\apjl 
\let\apjsupp=\apjs 
\let\applopt=\ao 





==> mjyu.tex <==
\def\nava{\leavevmode\hbox{,\kern-0.09em,}}%
\def\navb{\char'134}                                      %
\def\DJ{\leavevmode\setbox0=\hbox{D}\kern0pt
 \rlap{\kern.04em\raise.188\ht0\hbox{-}}D}
\def\dj{\leavevmode\setbox0=\hbox{d}\kern0pt
 \rlap{\kern.215em\raise.46\ht0\hbox{-}}d}
\def\SH{\v S} \def\sh{\v s} %
\def\CJ{\' C} \def\cj{\' c} %
\def\CH{\v C} \def\ch{\v c} %
\def\Z{\v Z} \def\z{\v z} %
\def\br{\break}



==> wncyr.tex <==
\def\rrmd{\font\tipo=wncyr12\tip}%
\def\rbfd{\font\tipo=wncyb12\tip}%
\def\rssd{\font\tipo=wncyss12\tip}%
\def\rrm{\font\tipo=wncyr10\tip}%
\def\rbf{\font\tipo=wncyb10\tip}%
\def\rit{\font\tipo=wncyi10\tip}%
\def\rss{\font\tipo=wncyss10\tip}%
\def\rsc{\font\tipo=wncysc10\tip}%
\def\rrmdev{\font\tipo=wncyr9\tip}%
\def\rbfdev{\font\tipo=wncyb9\tip}%
\def\ritdev{\font\tipo=wncyi9\tip}%
\def\rssdev{\font\tipo=wncyss9\tip}%
\def\rrmos{\font\tipo=wncyr8\tip}%
\def\rbfos{\font\tipo=wncyb8\tip}%
\def\ritos{\font\tipo=wncyi8\tip}%
\def\rssos{\font\tipo=wncyss8\tip}%
\def\rrmsev{\font\tipo=wncyr7\tip}%
\def\rbfsev{\font\tipo=wncyb7\tip}%
\def\ritsev{\font\tipo=wncyi7\tip}%
\def\tip{\relax\tipo\def\DD{\tipo\char'006}\def\dd{\tipo\char'016}%
\def\DJ{\DD}\def\dj{\dd}%
\def\ZZ{\tipo\char'021}\def\zz{\tipo\char'031}%
\def\Z{\ZZ}\def\z{\zz}%
\def\LJ{\tipo\char'001}\def\lj{\tipo\char'011}%
\def\NJ{\tipo\char'000}\def\nj{\tipo\char'010}%
\def\CC{\tipo\char'007}\def\cc{\tipo\char'017}%
\def\DZ{\tipo\char'002}\def\dz{\tipo\char'012}%
\def\XX{Q}\def\xx{q}%
\def\JJ{J}\def\jj{j}%
\def\SS{X}\def\ss{x}%
\def\JA{\tipo\char'027}\def\ja{\tipo\char'037}%
\def\SC{W}\def\sc{w}%
\def\CJ{\CC}\def\cj{\cc}%
\def\CH{Q}\def\ch{q}%
\def\SH{X}\def\sh{x}%
\def\EE{\tipo\char'003}\def\ee{\tipo\char'013}%
\def\JI{\tipo\char'022}\def\ji{\tipo\char'032}%
\def\JU{\tipo\char'020}\def\ju{\tipo\char'030}%
\def\M{\tipo\char'136}\def\m{\tipo\char'176}%
\def\TV{\tipo\char'137}\def\tv{\tipo\char'177}%
\def\rnava{\tipo\char'074}\def\rnavb{\tipo\char'076}%
\def\snava{\leavevmode\hbox{,\kern-0.06em,}}%
\def\snavb{\tipo\char'134}}%
\def\br{\break}%



